Hypergraph Contrastive Collaborative Filtering

Collaborative Filtering (CF) has emerged as fundamental paradigms for parameterizing users and items into latent representation space, with their correlative patterns from interaction data. Among various CF techniques, the development of GNN-based recommender systems, e.g., PinSage and LightGCN, has offered the state-of-the-art performance. However, two key challenges have not been well explored in existing solutions: i) The over-smoothing effect with deeper graph-based CF architecture, may cause the indistinguishable user representations and degradation of recommendation results. ii) The supervision signals (i.e., user-item interactions) are usually scarce and skewed distributed in reality, which limits the representation power of CF paradigms. To tackle these challenges, we propose a new self-supervised recommendation framework Hypergraph Contrastive Collaborative Filtering (HCCF) to jointly capture local and global collaborative relations with a hypergraph-enhanced cross-view contrastive learning architecture. In particular, the designed hypergraph structure learning enhances the discrimination ability of GNN-based CF paradigm, so as to comprehensively capture the complex high-order dependencies among users. Additionally, our HCCF model effectively integrates the hypergraph structure encoding with self-supervised learning to reinforce the representation quality of recommender systems, based on the hypergraph-enhanced self-discrimination. Extensive experiments on three benchmark datasets demonstrate the superiority of our model over various state-of-the-art recommendation methods, and the robustness against sparse user interaction data. Our model implementation codes are available at https://github.com/akaxlh/HCCF.

==> model.tex <==
% \section{Collaborative Filtering Paradigm}
\section{Preliminaries}
\label{sec:model}

% \subsection{Collaborative Filtering Paradigm}
We let $\mathcal{U}$ = $\{u_1,...,u_i,...,u_I\}$ ($|\mathcal{U}| = I$) and $\mathcal{V}$ = $\{v_1,...,v_j,...,v_J\}$ ($|\mathcal{V}| = J$) represent the set of users and items, respectively. The interaction matrix $\mathcal{A} \in \mathbb{R}^{I\times J}$ indicates the implicit relationships between each user in $\mathcal{U}$ and his/her consumed items. Each entry $\mathcal{A}_{i,j}$ in $\mathcal{A}$ will be set as 1 if user $u_i$ has adopted item $v_j$ before and $\mathcal{A}_{i,j}=0$ otherwise. The objective of CF task is to forecast the unobserved user-item interactions with the encoded corresponding representations. The assumption of CF paradigm lies in that behaviorally similar users are more likely to share similar interests. \\\vspace{-0.12in}

\noindent \textbf{Recap Graph-based Collaborative Filtering Paradigm}.
% Many existing CF approaches are designed with the various embedding functions to generate vectorized representations of users and items. Then, the similarity matching function is introduced to estimate the relevance score between user $u_i$ and the candiate item $v_j$. Following this paradigm, NCF~\cite{he2017neural} and DMF~\cite{xue2017deep} replaces the inner-product with Multilayer Perceptron to reconstruct the ground truth user-item interactions. Furthermore, To transform users and items into the latent embeddings, Autoencoder has been utilized as the embedding function with the behavior reconstruction objective, such as AutoRec~\cite{sedhain2015autorec} and CDAE~\cite{wu2016collaborative}.
In recent years, graph neural networks have been shown to be effective in learning representations over graph-structured data.
